Causal Impact of Masks, Policies, Behavior on Early Covid-19 Pandemic in the U.S

This paper evaluates the dynamic impact of various policies adopted by US states on the growth rates of confirmed Covid-19 cases and deaths as well as social distancing behavior measured by Google Mobility Reports, where we take into consideration people's voluntarily behavioral response to new information of transmission risks. Our analysis finds that both policies and information on transmission risks are important determinants of Covid-19 cases and deaths and shows that a change in policies explains a large fraction of observed changes in social distancing behavior. Our counterfactual experiments suggest that nationally mandating face masks for employees on April 1st could have reduced the growth rate of cases and deaths by more than 10 percentage points in late April, and could have led to as much as 17 to 55 percent less deaths nationally by the end of May, which roughly translates into 17 to 55 thousand saved lives. Our estimates imply that removing non-essential business closures (while maintaining school closures, restrictions on movie theaters and restaurants) could have led to -20 to 60 percent more cases and deaths by the end of May. We also find that, without stay-at-home orders, cases would have been larger by 25 to 170 percent, which implies that 0.5 to 3.4 million more Americans could have been infected if stay-at-home orders had not been implemented. Finally, not having implemented any policies could have led to at least a 7 fold increase with an uninformative upper bound in cases (and deaths) by the end of May in the US, with considerable uncertainty over the effects of school closures, which had little cross-sectional variation.

==> tables_and_figures/behavior-cases-nationinfo-pib.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & workplaces & retail & grocery & transit \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 masks for employees & 0.005 & 0.0005 & 0.003 & $-$0.010 \\ 
  & (0.008) & (0.015) & (0.011) & (0.023) \\ 
  closed K-12 schools & $-$0.044$^{***}$ & $-$0.025 & $-$0.069$^{**}$ & $-$0.047 \\ 
  & (0.013) & (0.018) & (0.027) & (0.041) \\ 
  stay at home & $-$0.034$^{***}$ & $-$0.047$^{***}$ & $-$0.071$^{***}$ & $-$0.074$^{***}$ \\ 
  & (0.011) & (0.013) & (0.015) & (0.028) \\ 
  business closure policies & $-$0.049$^{***}$ & $-$0.094$^{***}$ & $-$0.073$^{***}$ & $-$0.042 \\ 
  & (0.012) & (0.020) & (0.018) & (0.036) \\ 
  $\Delta \log \Delta C_{it}$ & 0.017$^{***}$ & 0.014$^{***}$ & 0.018$^{***}$ & 0.020$^{***}$ \\ 
  & (0.002) & (0.004) & (0.004) & (0.005) \\ 
  $\log \Delta C_{it}$ & $-$0.005 & $-$0.001 & 0.009 & 0.004 \\ 
  & (0.004) & (0.007) & (0.006) & (0.011) \\ 
  $\Delta \log \Delta C_{it}$.national & $-$0.033$^{***}$ & $-$0.086$^{***}$ & $-$0.018$^{**}$ & $-$0.053$^{***}$ \\ 
  & (0.005) & (0.008) & (0.008) & (0.012) \\ 
  $\log \Delta C_{it}$.national & $-$0.072$^{***}$ & $-$0.103$^{***}$ & $-$0.035$^{***}$ & $-$0.091$^{***}$ \\ 
  & (0.004) & (0.008) & (0.008) & (0.012) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.122$^{***}$ & -0.166$^{***}$ & -0.211$^{***}$ & -0.172$^{***}$ \\ 
 & (0.022) & (0.035) & (0.037) & (0.060) \\ 
Observations & 3,825 & 3,825 & 3,825 & 3,825 \\ 
R$^{2}$ & 0.953 & 0.906 & 0.765 & 0.856 \\ 
Adjusted R$^{2}$ & 0.952 & 0.905 & 0.764 & 0.855 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/behavior-cases-stateinfo-pib.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & workplaces & retail & grocery & transit \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 masks for employees & 0.023$^{*}$ & 0.033$^{*}$ & 0.012 & 0.015 \\ 
  & (0.012) & (0.020) & (0.012) & (0.025) \\ 
  closed K-12 schools & $-$0.196$^{***}$ & $-$0.253$^{***}$ & $-$0.143$^{***}$ & $-$0.243$^{***}$ \\ 
  & (0.030) & (0.048) & (0.027) & (0.050) \\ 
  stay at home & $-$0.028$^{**}$ & $-$0.024 & $-$0.068$^{***}$ & $-$0.062$^{**}$ \\ 
  & (0.013) & (0.017) & (0.015) & (0.028) \\ 
  business closure policies & $-$0.081$^{***}$ & $-$0.136$^{***}$ & $-$0.088$^{***}$ & $-$0.080$^{**}$ \\ 
  & (0.017) & (0.028) & (0.017) & (0.038) \\ 
  $\Delta \log \Delta C_{it}$ & 0.015$^{***}$ & $-$0.002 & 0.016$^{***}$ & 0.014$^{***}$ \\ 
  & (0.003) & (0.005) & (0.004) & (0.005) \\ 
  $\log \Delta C_{it}$ & $-$0.024$^{***}$ & $-$0.022$^{***}$ & $-$0.0002 & $-$0.018$^{*}$ \\ 
  & (0.005) & (0.008) & (0.005) & (0.010) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.282$^{***}$ & -0.380$^{***}$ & -0.287$^{***}$ & -0.371$^{***}$ \\ 
 & (0.041) & (0.066) & (0.040) & (0.078) \\ 
Observations & 3,825 & 3,825 & 3,825 & 3,825 \\ 
R$^{2}$ & 0.913 & 0.829 & 0.749 & 0.818 \\ 
Adjusted R$^{2}$ & 0.912 & 0.829 & 0.748 & 0.817 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/behavior-deathsinfo-nationinfo-pib.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & workplaces & retail & grocery & transit \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 masks for employees & 0.007 & 0.012 & 0.002 & $-$0.005 \\ 
  & (0.009) & (0.016) & (0.012) & (0.025) \\ 
  closed K-12 schools & $-$0.045$^{***}$ & $-$0.033$^{*}$ & $-$0.024 & $-$0.050 \\ 
  & (0.014) & (0.019) & (0.020) & (0.039) \\ 
  stay at home & $-$0.024$^{*}$ & $-$0.032$^{**}$ & $-$0.073$^{***}$ & $-$0.066$^{**}$ \\ 
  & (0.012) & (0.015) & (0.017) & (0.032) \\ 
  business closure policies & $-$0.044$^{***}$ & $-$0.091$^{***}$ & $-$0.067$^{***}$ & $-$0.054 \\ 
  & (0.012) & (0.021) & (0.020) & (0.039) \\ 
  $\Delta \log \Delta D_{it}$ & $-$0.003 & $-$0.012$^{***}$ & $-$0.002 & $-$0.009$^{*}$ \\ 
  & (0.002) & (0.004) & (0.004) & (0.005) \\ 
  $\log \Delta D_{it}$ & $-$0.007 & 0.003 & 0.002 & $-$0.0003 \\ 
  & (0.004) & (0.007) & (0.005) & (0.010) \\ 
  $\Delta \log \Delta D_{it}$.national & $-$0.058$^{***}$ & $-$0.095$^{***}$ & $-$0.008 & $-$0.067$^{***}$ \\ 
  & (0.005) & (0.008) & (0.006) & (0.010) \\ 
  $\log \Delta D_{it}$.national & $-$0.056$^{***}$ & $-$0.065$^{***}$ & $-$0.033$^{***}$ & $-$0.057$^{***}$ \\ 
  & (0.004) & (0.007) & (0.006) & (0.010) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.105$^{***}$ & -0.144$^{***}$ & -0.162$^{***}$ & -0.176$^{***}$ \\ 
 & (0.024) & (0.039) & (0.034) & (0.068) \\ 
Observations & 3,468 & 3,468 & 3,468 & 3,468 \\ 
R$^{2}$ & 0.953 & 0.899 & 0.783 & 0.856 \\ 
Adjusted R$^{2}$ & 0.953 & 0.898 & 0.782 & 0.855 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/behavior-deathsinfo-pib.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{8}{c}{\textit{Dependent variable:}} \\ 
\cline{2-9} 
 & workplaces & retail & grocery & transit & workplaces & retail & grocery & transit \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)\\ 
\hline \\[-1.8ex] 
 masks for employees & 0.018 & 0.027 & 0.006 & 0.006 & 0.019$^{*}$ & 0.029$^{*}$ & 0.006 & 0.011 \\ 
  & (0.011) & (0.017) & (0.014) & (0.026) & (0.010) & (0.017) & (0.013) & (0.025) \\ 
  closed K-12 schools & $-$0.226$^{***}$ & $-$0.261$^{***}$ & $-$0.114$^{***}$ & $-$0.240$^{***}$ & $-$0.224$^{***}$ & $-$0.254$^{***}$ & $-$0.117$^{***}$ & $-$0.238$^{***}$ \\ 
  & (0.024) & (0.033) & (0.018) & (0.035) & (0.027) & (0.039) & (0.020) & (0.041) \\ 
  stay at home & $-$0.031$^{**}$ & $-$0.035$^{**}$ & $-$0.082$^{***}$ & $-$0.072$^{**}$ & $-$0.033$^{**}$ & $-$0.041$^{**}$ & $-$0.080$^{***}$ & $-$0.076$^{**}$ \\ 
  & (0.012) & (0.017) & (0.016) & (0.031) & (0.014) & (0.018) & (0.018) & (0.032) \\ 
  business closure policies & $-$0.101$^{***}$ & $-$0.156$^{***}$ & $-$0.101$^{***}$ & $-$0.111$^{***}$ &  &  &  &  \\ 
  & (0.022) & (0.033) & (0.020) & (0.041) &  &  &  &  \\ 
  closed movie theaters &  &  &  &  & $-$0.015 & $-$0.021 & $-$0.025$^{*}$ & 0.035 \\ 
  &  &  &  &  & (0.017) & (0.020) & (0.015) & (0.028) \\ 
  closed restaurants &  &  &  &  & $-$0.049$^{***}$ & $-$0.084$^{***}$ & $-$0.034$^{**}$ & $-$0.087$^{**}$ \\ 
  &  &  &  &  & (0.018) & (0.024) & (0.014) & (0.040) \\ 
  closed non-essent bus &  &  &  &  & $-$0.033$^{**}$ & $-$0.044$^{**}$ & $-$0.041$^{***}$ & $-$0.044$^{*}$ \\ 
  &  &  &  &  & (0.014) & (0.017) & (0.015) & (0.026) \\ 
  $\Delta \log \Delta D_{it}$ & $-$0.012$^{***}$ & $-$0.031$^{***}$ & $-$0.001 & $-$0.021$^{***}$ & $-$0.012$^{***}$ & $-$0.029$^{***}$ & $-$0.001 & $-$0.019$^{***}$ \\ 
  & (0.005) & (0.006) & (0.004) & (0.006) & (0.004) & (0.006) & (0.004) & (0.006) \\ 
  $\log \Delta D_{it}$ & $-$0.013$^{***}$ & $-$0.001 & $-$0.005 & $-$0.006 & $-$0.014$^{***}$ & $-$0.003 & $-$0.005 & $-$0.008 \\ 
  & (0.004) & (0.006) & (0.005) & (0.009) & (0.004) & (0.007) & (0.005) & (0.009) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.340$^{***}$ & -0.425$^{***}$ & -0.292$^{***}$ & -0.417$^{***}$ & -0.335$^{***}$ & -0.415$^{***}$ & -0.292$^{***}$ & -0.400$^{***}$ \\ 
 & (0.026) & (0.036) & (0.033) & (0.060) & (0.026) & (0.038) & (0.033) & (0.060) \\ 
Observations & 3,468 & 3,468 & 3,468 & 3,468 & 3,468 & 3,468 & 3,468 & 3,468 \\ 
R$^{2}$ & 0.908 & 0.836 & 0.760 & 0.826 & 0.908 & 0.838 & 0.760 & 0.831 \\ 
Adjusted R$^{2}$ & 0.907 & 0.835 & 0.759 & 0.825 & 0.908 & 0.837 & 0.759 & 0.830 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{8}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/behavior-deathsinfo-stateinfo-pib.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & workplaces & retail & grocery & transit \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 masks for employees & 0.018 & 0.027 & 0.006 & 0.006 \\ 
  & (0.011) & (0.017) & (0.014) & (0.026) \\ 
  closed K-12 schools & $-$0.226$^{***}$ & $-$0.261$^{***}$ & $-$0.114$^{***}$ & $-$0.240$^{***}$ \\ 
  & (0.024) & (0.033) & (0.018) & (0.035) \\ 
  stay at home & $-$0.031$^{**}$ & $-$0.035$^{**}$ & $-$0.082$^{***}$ & $-$0.072$^{**}$ \\ 
  & (0.012) & (0.017) & (0.016) & (0.031) \\ 
  business closure policies & $-$0.101$^{***}$ & $-$0.156$^{***}$ & $-$0.101$^{***}$ & $-$0.111$^{***}$ \\ 
  & (0.022) & (0.033) & (0.020) & (0.041) \\ 
  $\Delta \log \Delta D_{it}$ & $-$0.012$^{***}$ & $-$0.031$^{***}$ & $-$0.001 & $-$0.021$^{***}$ \\ 
  & (0.005) & (0.006) & (0.004) & (0.006) \\ 
  $\log \Delta D_{it}$ & $-$0.013$^{***}$ & $-$0.001 & $-$0.005 & $-$0.006 \\ 
  & (0.004) & (0.006) & (0.005) & (0.009) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.340$^{***}$ & -0.425$^{***}$ & -0.292$^{***}$ & -0.417$^{***}$ \\ 
 & (0.026) & (0.036) & (0.033) & (0.060) \\ 
Observations & 3,468 & 3,468 & 3,468 & 3,468 \\ 
R$^{2}$ & 0.908 & 0.836 & 0.760 & 0.826 \\ 
Adjusted R$^{2}$ & 0.907 & 0.835 & 0.759 & 0.825 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/behavior-pib.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{8}{c}{\textit{Dependent variable:}} \\ 
\cline{2-9} 
 & workplaces & retail & grocery & transit & workplaces & retail & grocery & transit \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)\\ 
\hline \\[-1.8ex] 
 masks for employees & 0.023$^{*}$ & 0.033$^{*}$ & 0.012 & 0.015 & 0.024$^{**}$ & 0.035$^{*}$ & 0.012 & 0.018 \\ 
  & (0.012) & (0.020) & (0.012) & (0.025) & (0.012) & (0.020) & (0.012) & (0.024) \\ 
  closed K-12 schools & $-$0.196$^{***}$ & $-$0.253$^{***}$ & $-$0.143$^{***}$ & $-$0.243$^{***}$ & $-$0.195$^{***}$ & $-$0.242$^{***}$ & $-$0.147$^{***}$ & $-$0.238$^{***}$ \\ 
  & (0.030) & (0.048) & (0.027) & (0.050) & (0.031) & (0.050) & (0.028) & (0.051) \\ 
  stay at home & $-$0.028$^{**}$ & $-$0.024 & $-$0.068$^{***}$ & $-$0.062$^{**}$ & $-$0.029$^{**}$ & $-$0.031$^{*}$ & $-$0.065$^{***}$ & $-$0.065$^{**}$ \\ 
  & (0.013) & (0.017) & (0.015) & (0.028) & (0.015) & (0.018) & (0.017) & (0.029) \\ 
  business closure policies & $-$0.081$^{***}$ & $-$0.136$^{***}$ & $-$0.088$^{***}$ & $-$0.080$^{**}$ &  &  &  &  \\ 
  & (0.017) & (0.028) & (0.017) & (0.038) &  &  &  &  \\ 
  closed movie theaters &  &  &  &  & $-$0.007 & $-$0.004 & $-$0.016 & 0.049$^{*}$ \\ 
  &  &  &  &  & (0.014) & (0.019) & (0.014) & (0.027) \\ 
  closed restaurants &  &  &  &  & $-$0.040$^{***}$ & $-$0.088$^{***}$ & $-$0.031$^{**}$ & $-$0.079$^{**}$ \\ 
  &  &  &  &  & (0.015) & (0.020) & (0.012) & (0.037) \\ 
  closed non-essent bus &  &  &  &  & $-$0.029$^{**}$ & $-$0.033$^{*}$ & $-$0.039$^{***}$ & $-$0.033 \\ 
  &  &  &  &  & (0.013) & (0.017) & (0.013) & (0.023) \\ 
  $\Delta \log \Delta C_{it}$ & 0.015$^{***}$ & $-$0.002 & 0.016$^{***}$ & 0.014$^{***}$ & 0.016$^{***}$ & 0.001 & 0.016$^{***}$ & 0.018$^{***}$ \\ 
  & (0.003) & (0.005) & (0.004) & (0.005) & (0.003) & (0.005) & (0.004) & (0.005) \\ 
  $\log \Delta C_{it}$ & $-$0.024$^{***}$ & $-$0.022$^{***}$ & $-$0.0002 & $-$0.018$^{*}$ & $-$0.025$^{***}$ & $-$0.024$^{***}$ & $-$0.0001 & $-$0.020$^{**}$ \\ 
  & (0.005) & (0.008) & (0.005) & (0.010) & (0.005) & (0.008) & (0.005) & (0.010) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.282$^{***}$ & -0.380$^{***}$ & -0.287$^{***}$ & -0.371$^{***}$ & -0.276$^{***}$ & -0.363$^{***}$ & -0.285$^{***}$ & -0.348$^{***}$ \\ 
 & (0.041) & (0.066) & (0.040) & (0.078) & (0.042) & (0.067) & (0.040) & (0.076) \\ 
Observations & 3,825 & 3,825 & 3,825 & 3,825 & 3,825 & 3,825 & 3,825 & 3,825 \\ 
R$^{2}$ & 0.913 & 0.829 & 0.749 & 0.818 & 0.914 & 0.834 & 0.750 & 0.824 \\ 
Adjusted R$^{2}$ & 0.912 & 0.829 & 0.748 & 0.817 & 0.913 & 0.833 & 0.748 & 0.823 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{8}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-nosplit-pbiy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
 & \multicolumn{2}{c}{$\Delta \log \Delta C_{it}$} \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 lag(masks for employees, 14) & $-$0.090$^{***}$ & $-$0.100$^{***}$ \\ 
  & (0.031) & (0.029) \\ 
  lag(closed K-12 schools, 14) & $-$0.074 & 0.043 \\ 
  & (0.080) & (0.096) \\ 
  lag(stay at home, 14) & $-$0.063 & $-$0.079 \\ 
  & (0.050) & (0.052) \\ 
  lag(business closure policies, 14) & 0.051 & 0.045 \\ 
  & (0.062) & (0.060) \\ 
  lag(workplaces, 14) & 1.055$^{*}$ & 0.391 \\ 
  & (0.543) & (0.610) \\ 
  lag(retail, 14) & 0.594$^{*}$ & 0.316 \\ 
  & (0.303) & (0.316) \\ 
  lag(grocery, 14) & $-$0.471$^{*}$ & $-$0.259 \\ 
  & (0.284) & (0.282) \\ 
  lag(transit, 14) & 0.347 & 0.355 \\ 
  & (0.258) & (0.247) \\ 
  lag($\Delta \log \Delta C_{it}$, 14) & 0.015 & 0.024 \\ 
  & (0.026) & (0.028) \\ 
  lag($\log \Delta C_{it}$, 14) & $-$0.105$^{***}$ & $-$0.088$^{***}$ \\ 
  & (0.019) & (0.021) \\ 
  lag($\Delta \log \Delta C_{it}$.national, 14) &  & $-$0.095$^{**}$ \\ 
  &  & (0.042) \\ 
  lag($\log \Delta C_{it}$.national, 14) &  & $-$0.177$^{***}$ \\ 
  &  & (0.049) \\ 
  $\Delta \log T_{it}$ & 0.152$^{***}$ & 0.155$^{***}$ \\ 
  & (0.043) & (0.042) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.176 & -0.091 \\ 
 & (0.128) & (0.153) \\ 
$\sum_k w_k \mathrm{Behavior}_k$ & -0.804$^{***}$ & -0.425$^{***}$ \\ 
 & (0.140) & (0.157) \\ 
Observations & 3,825 & 3,825 \\ 
R$^{2}$ & 0.761 & 0.766 \\ 
Adjusted R$^{2}$ & 0.759 & 0.763 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-nosplit-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
 & \multicolumn{2}{c}{$\Delta \log \Delta C_{it}$} \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 lag(masks for employees, 14) & $-$0.083$^{**}$ & $-$0.103$^{***}$ \\ 
  & (0.038) & (0.033) \\ 
  lag(closed K-12 schools, 14) & $-$0.226$^{**}$ & 0.029 \\ 
  & (0.089) & (0.102) \\ 
  lag(stay at home, 14) & $-$0.127$^{**}$ & $-$0.115$^{**}$ \\ 
  & (0.057) & (0.054) \\ 
  lag(business closure policies, 14) & $-$0.076 & $-$0.001 \\ 
  & (0.068) & (0.061) \\ 
  lag($\Delta \log \Delta C_{it}$, 14) & 0.040 & 0.036 \\ 
  & (0.024) & (0.028) \\ 
  lag($\log \Delta C_{it}$, 14) & $-$0.137$^{***}$ & $-$0.091$^{***}$ \\ 
  & (0.022) & (0.026) \\ 
  lag($\Delta \log \Delta C_{it}$.national, 14) &  & $-$0.128$^{***}$ \\ 
  &  & (0.039) \\ 
  lag($\log \Delta C_{it}$.national, 14) &  & $-$0.243$^{***}$ \\ 
  &  & (0.045) \\ 
  $\Delta \log T_{it}$ & 0.156$^{***}$ & 0.158$^{***}$ \\ 
  & (0.044) & (0.042) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.512$^{***}$ & -0.190 \\ 
 & (0.150) & (0.156) \\ 
Observations & 3,825 & 3,825 \\ 
R$^{2}$ & 0.749 & 0.763 \\ 
Adjusted R$^{2}$ & 0.747 & 0.760 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-robust-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
 & \multicolumn{6}{c}{$\Delta \log \Delta C_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 lag(masks for employees, 14) & $-$0.083$^{**}$ & $-$0.078$^{**}$ & $-$0.059$^{*}$ & $-$0.079$^{**}$ & $-$0.075$^{**}$ & $-$0.060$^{*}$ \\ 
  & (0.038) & (0.039) & (0.031) & (0.034) & (0.035) & (0.035) \\ 
  lag(closed K-12 schools, 14) & $-$0.226$^{**}$ & $-$0.237$^{***}$ & $-$0.229$^{***}$ & $-$0.232$^{***}$ & $-$0.217$^{***}$ & $-$0.223$^{***}$ \\ 
  & (0.089) & (0.092) & (0.086) & (0.075) & (0.083) & (0.068) \\ 
  lag(stay at home, 14) & $-$0.127$^{**}$ & $-$0.132$^{**}$ & $-$0.127$^{**}$ & $-$0.096$^{*}$ & $-$0.110$^{**}$ & $-$0.100$^{*}$ \\ 
  & (0.057) & (0.058) & (0.056) & (0.056) & (0.051) & (0.054) \\ 
  lag(business closure policies, 14) & $-$0.076 & $-$0.077 & $-$0.080 & $-$0.044 & $-$0.095 & $-$0.073 \\ 
  & (0.068) & (0.069) & (0.067) & (0.061) & (0.067) & (0.061) \\ 
  lag(workplaces, 28) &  &  &  &  & $-$0.146 & 0.069 \\ 
  &  &  &  &  & (0.490) & (0.428) \\ 
  lag(retail, 28) &  &  &  &  & $-$0.303 & $-$0.415 \\ 
  &  &  &  &  & (0.356) & (0.358) \\ 
  lag(grocery, 28) &  &  &  &  & $-$0.227 & $-$0.396 \\ 
  &  &  &  &  & (0.250) & (0.255) \\ 
  lag(transit, 28) &  &  &  &  & 0.569$^{*}$ & 0.460 \\ 
  &  &  &  &  & (0.323) & (0.284) \\ 
  lag($\Delta \log \Delta C_{it}$, 14) & 0.040 & 0.034 & 0.038 & 0.042$^{*}$ & 0.042 & 0.044$^{*}$ \\ 
  & (0.024) & (0.024) & (0.024) & (0.024) & (0.028) & (0.026) \\ 
  lag($\log \Delta C_{it}$, 14) & $-$0.137$^{***}$ & $-$0.138$^{***}$ & $-$0.136$^{***}$ & $-$0.155$^{***}$ & $-$0.137$^{***}$ & $-$0.161$^{***}$ \\ 
  & (0.022) & (0.023) & (0.020) & (0.018) & (0.020) & (0.018) \\ 
  $\Delta \log T_{it}$ & 0.156$^{***}$ & 0.143$^{***}$ & 0.158$^{***}$ & 0.148$^{***}$ & 0.147$^{***}$ & 0.120$^{***}$ \\ 
  & (0.044) & (0.042) & (0.044) & (0.044) & (0.046) & (0.044) \\ 
  mask\_percent &  &  & $-$0.656 &  &  & $-$0.487 \\ 
  &  &  & (0.586) &  &  & (0.536) \\ 
  log(Trump voting shares) &  &  &  & 0.323$^{***}$ &  & 0.344$^{***}$ \\ 
  &  &  &  & (0.065) &  & (0.052) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.512$^{***}$ & -0.524$^{***}$ & -0.495$^{***}$ & -0.450$^{***}$ & -0.496$^{***}$ & -0.457$^{***}$ \\ 
 & (0.150) & (0.155) & (0.136) & (0.126) & (0.135) & (0.123) \\ 
Observations & 3,825 & 3,750 & 3,825 & 3,825 & 3,825 & 3,750 \\ 
R$^{2}$ & 0.749 & 0.746 & 0.751 & 0.757 & 0.752 & 0.758 \\ 
Adjusted R$^{2}$ & 0.747 & 0.743 & 0.749 & 0.755 & 0.749 & 0.756 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/deaths-deathsinfo-nosplit-pbiy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
 & \multicolumn{2}{c}{$\Delta \log \Delta D_{it}$} \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 lag(masks for employees, 21) & $-$0.146$^{***}$ & $-$0.147$^{***}$ \\ 
  & (0.050) & (0.049) \\ 
  lag(closed K-12 schools, 21) & $-$0.232$^{**}$ & $-$0.178$^{*}$ \\ 
  & (0.102) & (0.103) \\ 
  lag(stay at home, 21) & $-$0.066 & $-$0.065 \\ 
  & (0.067) & (0.067) \\ 
  lag(business closure policies, 21) & 0.098 & 0.107 \\ 
  & (0.087) & (0.092) \\ 
  lag(workplaces, 21) & 1.297$^{**}$ & 0.896 \\ 
  & (0.515) & (0.554) \\ 
  lag(retail, 21) & 0.572 & 0.523 \\ 
  & (0.441) & (0.438) \\ 
  lag(grocery, 21) & $-$0.935$^{**}$ & $-$0.887$^{**}$ \\ 
  & (0.388) & (0.368) \\ 
  lag(transit, 21) & 0.348 & 0.384 \\ 
  & (0.284) & (0.283) \\ 
  lag($\Delta \log \Delta D_{it}$, 21) & 0.016 & 0.016 \\ 
  & (0.035) & (0.037) \\ 
  lag($\log \Delta D_{it}$, 21) & $-$0.055$^{**}$ & $-$0.053$^{**}$ \\ 
  & (0.024) & (0.024) \\ 
  lag($\Delta \log \Delta D_{it}$.national, 21) &  & $-$0.034 \\ 
  &  & (0.044) \\ 
  lag($\log \Delta D_{it}$.national, 21) &  & $-$0.047 \\ 
  &  & (0.039) \\ 
   &  &  \\ 
  &  &  \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.346$^{**}$ & -0.283$^{*}$ \\ 
 & (0.162) & (0.172) \\ 
$\sum_k w_k \mathrm{Behavior}_k$ & -0.837$^{***}$ & -0.661$^{***}$ \\ 
 & (0.164) & (0.176) \\ 
Observations & 3,468 & 3,468 \\ 
R$^{2}$ & 0.518 & 0.518 \\ 
Adjusted R$^{2}$ & 0.512 & 0.513 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/deaths-deathsinfo-nosplit-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
 & \multicolumn{2}{c}{$\Delta \log \Delta D_{it}$} \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 lag(masks for employees, 21) & $-$0.134$^{***}$ & $-$0.156$^{***}$ \\ 
  & (0.051) & (0.050) \\ 
  lag(closed K-12 schools, 21) & $-$0.610$^{***}$ & $-$0.234$^{**}$ \\ 
  & (0.115) & (0.111) \\ 
  lag(stay at home, 21) & $-$0.082 & $-$0.068 \\ 
  & (0.066) & (0.066) \\ 
  lag(business closure policies, 21) & $-$0.059 & 0.059 \\ 
  & (0.086) & (0.086) \\ 
  lag($\Delta \log \Delta D_{it}$, 21) & $-$0.001 & 0.017 \\ 
  & (0.033) & (0.036) \\ 
  lag($\log \Delta D_{it}$, 21) & $-$0.078$^{***}$ & $-$0.064$^{**}$ \\ 
  & (0.026) & (0.027) \\ 
  lag($\Delta \log \Delta D_{it}$.national, 21) &  & $-$0.147$^{***}$ \\ 
  &  & (0.056) \\ 
  lag($\log \Delta D_{it}$.national, 21) &  & $-$0.116$^{***}$ \\ 
  &  & (0.032) \\ 
   &  &  \\ 
  &  &  \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.885$^{***}$ & -0.399$^{**}$ \\ 
 & (0.159) & (0.183) \\ 
Observations & 3,468 & 3,468 \\ 
R$^{2}$ & 0.502 & 0.512 \\ 
Adjusted R$^{2}$ & 0.497 & 0.507 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/deaths-robust-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
 & \multicolumn{6}{c}{$\Delta \log \Delta D_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 lag(masks for employees, 21) & $-$0.134$^{***}$ & $-$0.130$^{**}$ & $-$0.116$^{**}$ & $-$0.132$^{***}$ & $-$0.115$^{**}$ & $-$0.110$^{**}$ \\ 
  & (0.051) & (0.053) & (0.052) & (0.050) & (0.049) & (0.054) \\ 
  lag(closed K-12 schools, 21) & $-$0.610$^{***}$ & $-$0.615$^{***}$ & $-$0.611$^{***}$ & $-$0.617$^{***}$ & $-$0.596$^{***}$ & $-$0.592$^{***}$ \\ 
  & (0.115) & (0.118) & (0.113) & (0.107) & (0.119) & (0.112) \\ 
  lag(stay at home, 21) & $-$0.082 & $-$0.083 & $-$0.081 & $-$0.047 & $-$0.046 & $-$0.039 \\ 
  & (0.066) & (0.067) & (0.067) & (0.065) & (0.060) & (0.064) \\ 
  lag(business closure policies, 21) & $-$0.059 & $-$0.061 & $-$0.064 & $-$0.018 & $-$0.075 & $-$0.045 \\ 
  & (0.086) & (0.087) & (0.090) & (0.077) & (0.095) & (0.089) \\ 
  lag(workplaces, 35) &  &  &  &  & 1.170$^{*}$ & 1.313$^{**}$ \\ 
  &  &  &  &  & (0.611) & (0.544) \\ 
  lag(retail, 35) &  &  &  &  & $-$0.822$^{**}$ & $-$0.886$^{**}$ \\ 
  &  &  &  &  & (0.414) & (0.378) \\ 
  lag(grocery, 35) &  &  &  &  & 0.278 & 0.004 \\ 
  &  &  &  &  & (0.415) & (0.384) \\ 
  lag(transit, 35) &  &  &  &  & 0.095 & $-$0.070 \\ 
  &  &  &  &  & (0.258) & (0.232) \\ 
  lag($\Delta \log \Delta D_{it}$, 21) & $-$0.001 & $-$0.004 & $-$0.001 & 0.0001 & $-$0.020 & $-$0.013 \\ 
  & (0.033) & (0.035) & (0.033) & (0.032) & (0.040) & (0.042) \\ 
  lag($\log \Delta D_{it}$, 21) & $-$0.078$^{***}$ & $-$0.073$^{***}$ & $-$0.077$^{***}$ & $-$0.093$^{***}$ & $-$0.065$^{**}$ & $-$0.077$^{***}$ \\ 
  & (0.026) & (0.027) & (0.024) & (0.022) & (0.026) & (0.024) \\ 
  mask\_percent &  &  & $-$0.510 &  &  & $-$0.338 \\ 
  &  &  & (0.476) &  &  & (0.450) \\ 
  log(Trump voting shares) &  &  &  & 0.356$^{***}$ &  & 0.337$^{***}$ \\ 
  &  &  &  & (0.073) &  & (0.077) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.885$^{***}$ & -0.889$^{***}$ & -0.871$^{***}$ & -0.815$^{***}$ & -0.832$^{***}$ & -0.785$^{***}$ \\ 
 & (0.159) & (0.163) & (0.147) & (0.146) & (0.160) & (0.154) \\ 
Observations & 3,468 & 3,400 & 3,468 & 3,468 & 3,468 & 3,400 \\ 
R$^{2}$ & 0.502 & 0.492 & 0.503 & 0.511 & 0.505 & 0.504 \\ 
Adjusted R$^{2}$ & 0.497 & 0.487 & 0.498 & 0.506 & 0.500 & 0.498 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/policy-ip.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
 & masks for employees & closed K-12 schools & stay at home & business closure policies & masks for employees & closed K-12 schools \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 lag(workplaces, 14) & $-$0.057 & $-$0.058 & 0.443 & 0.411 & $-$0.050 & 0.002 \\ 
  & (0.680) & (0.096) & (0.571) & (0.403) & (0.757) & (0.098) \\ 
  lag(retail, 14) & 0.418 & $-$0.056 & $-$0.987$^{*}$ & $-$1.609$^{***}$ & $-$0.089 & 0.218$^{*}$ \\ 
  & (0.656) & (0.130) & (0.548) & (0.316) & (0.723) & (0.113) \\ 
  lag(grocery, 14) & $-$0.112 & 0.093 & $-$0.095 & 0.353 & 0.424 & $-$0.213 \\ 
  & (0.427) & (0.164) & (0.439) & (0.242) & (0.527) & (0.157) \\ 
  lag(transit, 14) & $-$0.504 & $-$0.087$^{*}$ & $-$0.412 & 0.142 & $-$0.614 & $-$0.026 \\ 
  & (0.416) & (0.046) & (0.346) & (0.256) & (0.415) & (0.037) \\ 
  $\Delta \log \Delta C_{it}$ & $-$0.096$^{***}$ & $-$0.018 & $-$0.016 & $-$0.025 & $-$0.119$^{***}$ & $-$0.003 \\ 
  & (0.029) & (0.015) & (0.036) & (0.018) & (0.032) & (0.015) \\ 
  $\log \Delta C_{it}$ & 0.023 & 0.012 & 0.036 & 0.043$^{**}$ & 0.038 & 0.004 \\ 
  & (0.034) & (0.009) & (0.024) & (0.017) & (0.036) & (0.009) \\ 
  $\Delta \log \Delta C_{it}$.national &  &  &  &  & $-$0.059 & 0.005 \\ 
  &  &  &  &  & (0.098) & (0.026) \\ 
  $\log \Delta C_{it}$.national &  &  &  &  & $-$0.319$^{***}$ & 0.162$^{***}$ \\ 
  &  &  &  &  & (0.077) & (0.023) \\ 
  log(Trump voting shares) & 0.004 & 0.021 & $-$0.252$^{**}$ & $-$0.145$^{**}$ & 0.009 & 0.015 \\ 
  & (0.109) & (0.046) & (0.104) & (0.070) & (0.100) & (0.044) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Behavior}_j$ & 0.084 & 0.074 & 0.415$^{**}$ & 0.388$^{***}$ & 0.269 & -0.052 \\ 
 & (0.198) & (0.054) & (0.188) & (0.100) & (0.275) & (0.055) \\ 
Observations & 3,825 & 3,825 & 3,825 & 3,825 & 3,825 & 3,825 \\ 
R$^{2}$ & 0.534 & 0.220 & 0.585 & 0.603 & 0.548 & 0.273 \\ 
Adjusted R$^{2}$ & 0.530 & 0.213 & 0.582 & 0.599 & 0.544 & 0.266 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
